Lovelock gravity, black holes and holography

This thesis is divided in two separate parts, the first concerned with gravitational aspects of Lovelock theories, the second with some of their holographic applications.

==> ShockW.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Shock waves in higher curvature gravity}
\label{SW}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\comment{Applications! numericalGR testbed, heavy ion collisions, holography, etc.}


\noindent
Another very interesting (and simple) class of solutions is that of shock waves (or pp-waves) that are solutions of higher curvature gravity theories independently of the corrections included, Lovelock or not. These solutions will be extensively used in some parts of the thesis. These will be useful in order to analyze the causal structure of these theories. 

Particularity that they are not corrected by any

\begin{itemize}
\item Shock waves in asymptotically flat and AdS spacetimes
\item Higher curvature corrections
\item Massless fields in AdS spacetimes
\item Probing shock waves in general gravity theories
\end{itemize}

\comment{Meter tesoiras!!}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Massless fields in AdS spacetime}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A much more suitable background for the kind of computation we are performing is the shock wave discussed by Horowitz and Itzhaki and that corresponds to a massless field in AdS. The coordiante system for AdS chosen for that purpose makes much more clear the analogy with the flat case as it makes manifest how AdS is conformally related to the flat metric. 
%
\begin{equation}
d\hat{s}^2=\frac{4\eta_{\mu\nu}dx^{\mu}dx^{\nu}}{(1-\eta_{\alpha\beta}x^\alpha x^\beta)^2}
\end{equation}
%
where we will be considering null coordinates, $x^{\mu}=(u,v,x^i)$.
Remark that this metric is non-static and that the null vector $l^\mu=\delta^\mu_v$ is not in general Killing, just for $u=0$ that will be the chosen position of our shock wave. In general $l^\mu$ is just a conformal Killing vector. 

We can write the connection in terms of a new vector $V^\mu$, proportional to $x^{\mu}$ in this case, as,
%
\begin{equation}
\hat{\Gamma}^{\mu}_{\alpha \beta}=-\left[V_\alpha\delta^{\mu}_\beta+V_\beta\delta^{\mu}_\alpha-V^{\mu}\hat{g}_{\alpha\beta}\right]
\end{equation}
%
in such a way that 
%
\begin{equation}
\hat{\nabla}_{(\alpha}l_{\beta)}=-2(V\cdot l)\hat{g}_{\alpha\beta}\sim u \hat{g}_{\alpha\beta}
\end{equation}
%
one can think of constructing a Killing vector in the neighbourhood of $u=0$ as a power series: $\tilde{l}^\mu=l^\mu+u A^{\mu}(x^i)+\ldots$ The ansatz for the shock wave is 
%
\begin{equation}
g_{\mu\nu}=\hat{g}_{\mu\nu}+\delta(u) F(x^i)l_\mu l_\nu
\end{equation}
%
the $\delta$-function basically kills all the u-dependence of the shock wave term in such a way that it would be equivalent to consider the Killing vector. For practical purposes it will equivalent to consider the $l$-vector itself Killing for all what concerns the shock wave. The total connection can be written as 
%
\begin{equation}
\Gamma^\mu_{\alpha\beta}=\hat{\Gamma}^\mu_{\alpha\beta}+\left[(K_\alpha l_\beta+K_\beta l_\alpha)l^\mu-\tilde{K}^\mu l_\alpha l_\beta\right]
\end{equation}
%
where $K_\mu l^\mu=\tilde{K}_\mu l^\mu=0$ in such a way that 
%
\begin{equation}
\nabla_\alpha l_\beta= \hat{\nabla}_\alpha l_\beta=-2V_{[\alpha} l_{\beta]}
\label{killing}
\end{equation}
%
and the Killing condition is the same for the full metric as for the AdS term. 

The Riemman tensor can be written as
%
\begin{equation}
R_{\mu\nu\alpha\beta}=-\left(g_{\mu\alpha}g_{\nu\beta}-g_{\mu\beta}g_{\nu\alpha}\right)+\check{R}_{\mu\nu\alpha\beta}
\end{equation}
%
where the extra term has a very simple expression in terms of $l^\mu$
%
\begin{equation}
\check{R}_{\mu\nu\alpha\beta}=l_{[\mu}K_{\nu][\alpha}l_{\beta]}
\end{equation}
%
where $K_{\mu\nu}$ is a symmetric tensor made from $F$ its derivatives and $V^{\mu}$ verifying
%
\begin{equation}
K_{\mu\nu}l^{\nu}=0
\end{equation}
%
Notice that $K_\mu$, $\tilde{K}_\mu$ and $K_\mu\nu$ are proportional to $\delta(u)$ in such a way that they are zero when multiplied by $u$. 
The last property just follows from $(\nabla_{\alpha}\nabla_{\beta}-\nabla_{\beta}\nabla_{\beta})l_\nu=R_{\mu\nu\alpha\beta}\, l^{\mu}$ that because of the previous properties has to be equal to $(\hat{\nabla}_{\alpha}\hat{\nabla}_{\beta}-\hat{\nabla}_{\beta}\hat{\nabla}_{\beta})l_\nu=\hat{R}_{\mu\nu\alpha\beta}\, l^{\mu}$ in such a way that $\check{R}_{\mu\nu\alpha\beta}\, l^{\mu}=0$.

All these properties are shared by shock waves in other coordinate patches of AdS where the analysis is much simpler $l^\mu$ being an exact Killing vector everywhere.

The form of expressing the Riemman tensor is particularly useful to discuss the equations of motion for this type of backgrounds. The AdS background is a solution of the Einstein equations with cosmological constant
%
\begin{equation}
R_{\mu\nu}=-(d-1)g_{\mu\nu}
\end{equation}
%
in such a way that in order for the shock wave solution to be also a solution it must verify
%
\begin{equation}
K^\mu_{\ \ \mu}=0
\label{SWeq}
\end{equation}
%
which is a linear equation for $F$ is such a way that we can construct new solutions by superposing simpler ones. 
Horowitz and Itzhaki have proven that this solution is not corrected when higher curvature corrections are included. Let me discuss here their argument as it will be useful for the discussion of the equations of motion for perturbations. We will closely follow the approach of Frolov et al. First we will consider scalars made just from the metric and the Riemman tensor. Their contibution can be organized in powers of the extra piece of the Riemman $\check{R}$ that contains two $l^\mu$ that have to be contracted with either another $l^\mu$ or $K_{\mu\nu}$. In any case the term necessarily vanishes. 

In order to include covariant derivatives we will make use of the fact that $l^\mu$ is a null Killing vector orthogonal to all the tensors that can be constructed from the metric. We will denote by $S_n$ a given scalar with $n$ covariant derivatives. The degree $n$ of a given scalar can be reduced following two steps. 

\begin{itemize}
\item If the given term contains $\nabla_{\alpha}l_\beta$ we can eliminate the covariant derivative by using (\ref{killing}) untill we eliminate all covariant derivatives acting on it. The resulting scalar necessarily has lower degree than the original one.

\item  For a general scalar, $l^\mu$ has to be contracted either with one of the available tensors $F$, $l^\mu$, $V^\mu$ and $K_{\mu\nu}$, or any of the covariant derivatives. We can again make use of the Killing equation in order to conmute the vector $l^\mu$ with the covariant derivatives without increasing the degree of the scalar, using
%
\begin{equation}
l_\alpha \nabla_\beta(\cdots)=\nabla_\beta[l_\alpha(\cdots)]+2V_{[\beta}l_{\alpha]}(\cdots)
\label{commute}
\end{equation}
%
then we can reduce all possible scalars to two possible kinds of terms depending on where the $l^\mu$ is contracted. We may have either
%
\begin{equation}
\nabla\cdots\nabla[l^\alpha\nabla_\alpha(\cdots)] \qquad \text{or} \qquad \nabla\cdots\nabla[l^\alpha T_{\ldots \,\alpha \ldots}(\cdots)]
\end{equation}
%
contracted with some other tensor with the necessary number of indices to construct the scalar. The first term vanishes because the quantity inside the square brackets is just the Lie derivative with respect to the Killing vector of some vector that of course vanishes. The second term is also zero as any of the available tensors is orthogonal to $l^\mu$.
\end{itemize}

In this way we can reduce the degree of the initial scalar util we a scalar without any covariant derivative which, as discussed before, necessarily vanishes.
Thus, any scalar made from the metric, the Riemman tensor and its covariant derivatives, containing at least one power of $\check{R}$ is zero off-shell as we did not need to impose (\ref{SWeq}) on any step. The only 

We can also verify that the only (0,2)-tensor containing at least one power of $\check{R}$  that is non-vanishing off-shell is the Ricci tensor. In this kind of terms we have at least two $l^\mu$ factors that can either be contracted as discussed in the previus section or free. If it is not contracted with anything we can again use the property (\ref{commute}) to put it in front as a global factor. If it is contracted we can use the same steps discussed above to reduce the degree of the tensor until it either has no covariant derivatives, in which case if the $l^\mu$ is contracted necessarily vanishes, or the Killing vector is no longer contracted in which case we can again put it as a global factor. We can perform the same type operations for the other $l^\mu$ in such a way that the only non-vanishing terms will be of the form $l_\alpha l_\beta$ times some scalar made from everything else. This scalar however cannot contain any further $l^\mu$ and thus terms linear in $\check{R}$ contribute.

There are two such terms we can form, one is the Ricci tensor
%
\begin{equation}
\check{R}_{\mu\nu}=-\frac14 K^\alpha_{\ \ \alpha}l_{\mu}l_\nu
\end{equation}
%
and once this is set to zero we are left just with,
%
\begin{equation}
\nabla^\alpha\nabla^\beta\check{R}_{\alpha\mu\beta\nu}=\nabla^2 \check{R}_{\mu\nu}-\nabla^\alpha\nabla_{\mu}\check{R}_{\alpha\nu}
\end{equation}
%
that necessarily vanishes because of the Bianchi identity and the fact that $\check{R}_{\mu\nu}=0$ on-shell. Thus just the Einstein-Hilbert term contributes to the equation of motion for the shock wave, all the other give a contribution proportional to this ({\it e.g.} Lovelock gravities) or just involving the metric, thus just {\it renormalizing} the value of the cosmological constant. In particular, the equation of motion would be the same even if we consider that the AdS any of the AdS vacua of Lovelock theories (or any higher curvature gravity in general) distinct from the Einstein-Hilbert one. 

Another useful property of the background metric is that,
%
\begin{equation}
\nabla^2 \check{R}_{\mu\nu\alpha\beta}\sim \check{R}_{\mu\nu\alpha\beta}+ \mathcal{O}(\check{R}^2)
\end{equation}
%
again because of the Bianchi identity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Probing shock waves in general theories of gravity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We will now analyze which terms contribute to the equation of motion for perturbations in the large momentum regime. For that we will have to restrict to theories that yield two derivative equations of motion for the perturbations about the shock wave background (and AdS), at least up to dimension six terms. 

We will see that to that order just the three point function matters in the sense that the only terms that enter the equations of motion for perturbations about the shock wave background are those contributing to $t_{2,4}$ the parameters in the energy one point function in a state created by the stress energy tensor. These is also consistent with field redefinition analysis of the independent terms in the action. Higher dimension terms of the form $R^2\nabla^{2n} R$ also contribute and most probably they parametrize the higher derivative contributions to the equations of motion for perturbations.  

Before however it is instructive to analyze what happens for bosonic fields of lower spin. If we consider a minimally coupled scalar in this background its equation of motion will just be
%
\begin{equation}
\nabla^2\phi=0
\end{equation}
%
where we consider $\phi$ as a small perturbation in such a way that we do not need to consider backreaction (we could also include $\phi$ as a source for the shock wave itself). In the large momentum limit considering just terms yielding two derivative equations of motion for $\phi$ in the action we have to consider terms like
%
\begin{equation}
\mathcal{H}^{\mu\nu}\nabla_\mu\nabla_\nu\phi
\end{equation}
%
where the tensor $\mathcal{H}$ is just made from the background metric, Riemann and covariant derivatives. However we already saw that there is no (2,0)-tensor that is not vanishing on-shell. Thus such terms do note exist and the linear equation for the scalar is not corrected at the two derivative level. 

The same happens for a vector field $A_\mu$. The Maxwell equations 
%
\begin{equation}
\nabla^\mu F_{\mu\nu}=0
\end{equation}
%
will be corrected in the high momentum limit at the two derivative level by terms of the form
%
\begin{equation}
\mathcal{H}^{\mu\nu\alpha\beta}\nabla_\nu F_{\alpha\beta}
\end{equation}
%
where again $\mathcal{H}$ is a background tensor. In principle, applying the same procedure discussed in the previous section, this tensor can be at most quadratic in $\check{R}$ as it has four indices and each of them can accomodate one factor $l^\mu$. In the quadratic case then $\mathcal{H}_{\mu\nu\alpha\beta}=Hl_\mu l_\nu l_\alpha l_\beta$ but $F_{\alpha\beta}$ is antisymmetric in its two indices in such a way that $l^{\alpha}l^\beta\nabla F_{\alpha\beta}=0$ and the term above vanishes. We are left with terms linear in $\check{R}$ and taking into account
%
\begin{equation}
\nabla^2 \check{R}_{\mu\nu\alpha\beta}\sim \check{R}_{\mu\nu\alpha\beta} \qquad \text{and} \qquad \nabla^\mu \check{R}_{\mu\nu\alpha\beta}=0
\end{equation}
%
and that at the linear level we can commute covariant derivatives, we just have to consider tensors
%
\begin{equation}
\nabla_{\alpha_1}\cdots \nabla_{\alpha_n}\check{R}_{\beta_1 \cdots \beta_4}
\end{equation}
%
without contracting any indices otherwise yielding zero or reduzing to another term of the same type. The number of free indices is bounded to beequal or less than four and then we cannot include any covariant derivative. The only extra contribution to the equation of motion of the vector field is then
%
\begin{equation}
\check{R}^{\mu\nu\alpha\beta}\nabla_\nu F_{\alpha\beta}
\end{equation}
%
that is the high momentum limit of $\nabla_\nu(\check{R}^{\mu\nu\alpha\beta}F_{\alpha\beta})$ that arise from a $\check{R}^{\mu\nu\alpha\beta}F_{\mu\nu}F_{\alpha\beta}$

In both cases the possible contributions to the perturbation equations are in one to one correspondence with the possible energy one point functions that is the same as the 3-point functions of a graviton with two either scalar or vectors. In the vector case the coefficient of the extra term is proportional to the the adimensional $a_2$ coefficient appearing in the energy one point function of a state created by a conserved current. If we parameterize the equation of motion for the perturbation as 
%
\begin{equation}
\nabla^{\mu}F_{\mu\nu} + \alpha_2\, \check{R}_{\nu}^{\ \ \mu\alpha\beta}\nabla_\mu F_{\alpha\beta} = 0
\end{equation}
%
the relation of $\alpha_2$ and $a_2$ is
%
\begin{equation}
a_2 = -6 \alpha_2
\end{equation}
%

The expectation is that the same should happen also for graviton 3-point functions. One should be able to find three possible structures corresponding to the Einstein-Hilbert contribution (isotropic), the one appearing in Lovelock theories ($t_2$) and another one ($t_4$).

Again, in the high momentum limit at two derivative level, the possible extra contributions are of the form,
%
\begin{equation}
\mathcal{H}^{\mu\nu\alpha\beta\rho\sigma}\;\delta R_{\alpha\beta\rho\sigma}
\end{equation}
%
We have six slots in $\mathcal{H}$ in order to have up to six $l^\mu$ vectors so in principle we have to consider up to cubic terms in $\check{R}$. The cubic terms however do not give any contribution because of a similar reason as for the vanishing of quadratic terms for vector perturbations. $l^\mu l^\nu \delta R_{\mu\nu\alpha\beta}=0$ because of the antisymmetry of the first pair of indices. 

The Einstein-Hilbert contribution is 
%
\begin{equation}
\delta R_{\mu\nu}\sim \nabla^2 h_{\mu\nu}
\end{equation}
%
when we choose the transverse traceless gauge, $\nabla^\mu h_{\mu\nu}=h^\alpha_{\ \ \alpha}=0$. This is the only possible $\mathcal{O}(\check{R}^0)$ term. Then the full equation will correspond to that plus higher order terms in such a way that we can trade $\delta R_{\mu\nu}$ by those higher order terms. The possible quadratic $\mathcal{H}$ tensors are of the form
%
\begin{equation}
(\nabla_{\alpha_1}\cdots\nabla_{\alpha_n} \check{R}_{\gamma_1\cdots\gamma_4})(\nabla_{\beta_1} \cdots \nabla_{\beta_m} \check{R}_{\lambda_1\cdots\lambda_4})g_{\cdots}\cdots g_{\cdots}
\end{equation}
% 
where the pairs of indices cannot be contracted inside the brackets and we have to have at least four free indices in order to accomodate the four $l^\mu$. %The only way to accomodate all that is with 
%
%\begin{equation}
%\mathcal{H}=(\nabla_{\alpha_1}\cdots\nabla_{\alpha_n} \check{R}_{\gamma_1\cdots\gamma_4})(\nabla_{\beta_1} \cdots \nabla_{\beta_m} \check{R}_{\lambda_1\cdots\lambda_4})
%\end{equation}
%
%with all indices from one pair of brackets contracted with those in the other leaving six free. This imply that we either have one of four possibilities. Considering $n\geq m$, more precisely $n=m+2p$ we will have 3+p free indices in the first bracket and 3-p in the second, for $p=0,1,2,3$ and then all possible different ways of contracting these tensors with $\delta R_{\mu\nu\alpha\beta}$. It seems like too many possibilities...
Any of them ends up being of the form
%
\begin{equation}
l_\mu l_\nu \;S(\nabla, F, V_\alpha, K_{\alpha\beta}, L_{\alpha\beta}) 
\end{equation}
%
where $S(\cdots)$ is a scalar made of the indicated elements, $L$ being
%
\begin{equation}
L_{\mu\nu}=\delta R_{\mu\alpha\nu\beta}\;l^\alpha l^\beta
\end{equation}
%
in such a way that $L^\mu_{\ \mu}=L_{\mu\nu}l^{\nu}=0$. Then, all quadratic terms just contribute to $\mathcal{E}_{uu}$ thus just to the helicity zero case. Even in that case one has to check that the equations of motion are consistent otherwise one should discard these terms. 

For instance if we add these terms alone to the Einstein-Hilbert action we would get in the high momentum limit
%
\begin{equation}
\partial^\mu\partial_\mu h_{uu}+\gamma (\cdots) =0
\end{equation}
%
but $h_{uu}$ is zero in the transverse gauge if we consider the incoming wave direction $P_v$. Then unless the terms in brackets are zero, the coefficient $\gamma$ would have to be necessarily zero.

%Terms quadratic in $\check{R}$ come from quartic terms in the action and higher and terms with covariant derivatives. 

%Thus, these contribute to 4-point functions and higher. Maybe assuming something else (symmetry?) about the background solution some of them vanish. Considering a `small' shock wave maybe we can consider them subleading. 


The linear terms are much simpler. In this case we have just
%
\begin{equation}
\check{R}_{(\mu}^{\ \ \rho\alpha\beta}\delta R_{\nu)\rho\alpha\beta} \qquad \text{or} \qquad (\nabla\nabla \check{R})^{\mu\nu\alpha\beta\rho\sigma}\;\delta R_{\alpha\beta\rho\sigma}
\end{equation}
%
We could also include terms in $\delta R_{\mu\nu}$ but these would reduce to quadratic terms when the equation of motion is imposed. Also the covariant derivative indices in the second term are symmetric as the antisymmetric part reduces to the first term plus a quadratic contribution. There is only one independent way of contracting the indices in the second kind of term
%
\begin{equation}
\left[\nabla_{(\mu}\nabla_{\nu)}\check{R}^{\alpha\beta\rho\sigma}\right]\delta R_{\alpha\beta\rho\sigma}
\end{equation}
%
all other possible terms are related to this one via the Bianchi identity and the symmetries of $\delta R$ plus maybe some quadratic terms.

These two terms exactly correspond to the two extra (in addition to the isotropic one from the Einstein-Hilbert term) possible structures appearing in the three point function of gravitons. The coefficients of both terms contribute to $t_2$ and that of the second to $t_4$. This can be easily checked computing the energy one point function for a $h_{12}$ perturbation as in CCP to obtain
%
\begin{eqnarray}
\check{R}_{(\mu}^{\ \ \rho\alpha\beta}\delta R_{\nu)\rho\alpha\beta} & \sim & \left(\frac{n_1^2+n_2^2}{2}-\frac1{d-2}\right)\equiv T_2 \\
\left[\nabla_{(\mu}\nabla_{\nu)}\check{R}^{\alpha\beta\rho\sigma}\right]\delta R_{\alpha\beta\rho\sigma} & \sim & \left(2n_1^2 n_2^2-\frac2{d(d-2)}\right) + \#  T_2
\end{eqnarray}
%
that exacyly correspond to the $t_{2,4}$ structures in the energy one point function. If we parametrize the equation of motion for perturbations as 
%
\begin{equation}
\delta R_{\mu\nu} + 2 \gamma_2 \; \check{R}_{(\mu}^{\ \ \rho\alpha\beta}\delta R_{\nu)\rho\alpha\beta} + 2 \gamma_4 \; [\nabla_{(\mu}\nabla_{\nu)}\check{R}^{\alpha\beta\rho\sigma}]\delta R_{\alpha\beta\rho\sigma}=0
\end{equation}
%
in five dimensions the relation to the energy one point function parameters is
%
\begin{equation}
t_2=24(36\gamma_4 -\gamma_2) \qquad  \qquad t_4=-1440\gamma_4
\end{equation}
%

These terms are in one to one correspondence to the independent contributions to the effective action under field redefinitions. In flat space we know that (at least up to cubic order {\it i.e} dimension six terms) the coefficients of terms containing the Ricci tensor are ambiguous in the sense that they can be fixed freely by a general field redefinition. In AdS the analysis can be performed in exactly the same way if we write the action in terms of 
%
\begin{equation}
\check{R}_{\mu\nu\alpha\beta}=R_{\mu\nu\alpha\beta}+2g_{\mu[\alpha}g_{\beta]\nu}
\end{equation}
%
and organize all terms depending on the order in $\check{R}$. Then on Einstein-shell
%
\begin{equation}
\check{R}_{\mu\nu}=0
\end{equation}
%
(or more generally $\check{R}_{\mu\nu}\sim \mathcal{O}(\check{R}^2)$) and we can use a general field redefinition
%
\begin{equation}
\tilde{g}_{\mu\nu}\rightarrow g_{\mu\nu}+\alpha_1\; \check{R}_{\mu\nu}+\alpha_2\; \check{R}\; g_{\mu\nu} + \mathcal{O}(\check{R}^2)
\end{equation}
%
as the new tensor is just the Weyl tensor on Einstein shell and the analysis carries over as in asymptotically flat spacetimes. 

Then, up to dimension six we have just four possible independent contributions, the Einstein-Hilbert term, a quadratic contribution that can be chosen as the Gauss-Bonnet term, and two cubic terms. One of the cubic terms can be chosen to be the cubic Lovelock lagrangian while the other one can be chosen to be 
%
\begin{equation}
\mathcal{I}_3=R^{\mu\nu}_{\ \ \alpha\beta}R^{\alpha\beta}_{\ \ \rho\sigma}R^{\rho\sigma}_{\ \ \mu\nu}+\ldots
\end{equation}
%
where the dots stand for terms containing the Ricci in such a way that the equation of motion for perturbations about the shock wave background is second order [Is that possible??]. Both of the Lovelock combinations contribute to in the same way, just to $t_2$. Whereas the $t_4$ contribution comes solely from $\mathcal{I}_3$. In a way this analysis is insinuating that all terms yielding for instance
%
\begin{equation}
\check{R}_{\alpha\beta\rho\sigma}\nabla_{(\mu}\nabla_{\nu)}\delta R^{\alpha\beta\rho\sigma}
\end{equation}
%
are ambiguous and can be removed by field redefinitions. These term is dimension six but we have just seen that the independent order six contributions to the action are already accounted for by the terms contributing to $t_{2,4}$.  

As discussed before terms with more than four $\check{R}$ in the action are not relevant for our analysis as they would be quadratic in $\check{R}$ in the equations for the metric perturbations and so do not contribute. But there still room for higher derivative contributions parametrized by terms type $\check{R}^2\nabla^{2n} \check{R}$. In the high momentum limit these terms would be leading however if they contribute to the time delay with different sign for two different helicities of the graviton they would ruled out in the same way as $t_{2,4}$ (see below). [higher point functions?]

Analyzing the collision of perturbations in the shock wave background of Horowitz and Itzhaki we find the same type of causality violation as analyzed in previous sections. In five dimensions the profile can be found to be
%
\begin{equation}
F(r)=\frac{\alpha(r-1)^4}{r(1-r^2)^2}
\end{equation}
%
where $\alpha$ is related to the energy of the shock and we have chosen the profile so that it vanishes at the boundary, $r=1$.

For the helicity two graviton the time delay is proportional to
%
\begin{equation}
\Delta_2= 1 - \frac{(1+r_0)^4}{48 r_0^2} t_2 + \frac{(1+r_0)^4(1-10 r_0^2 + r_0^4)}{960 r_0^4} t_4
\end{equation}
%
where we translated the $\gamma_{2,4}$ dependence into $t_{2,4}$. Then $\Delta_2\geq 0$ then translates into a constraint on these two parameters. Remarkably this constraint coincides with the one coming from positivity of the energy! And then rules out a bigger and bigger part of the parameter space as we explore smaller values for the impact parameter $r_0$. 

Something similar happens for the helicity one graviton (even though the constraint does not coincide with the one from positivity, meybe because of a mistake) 
%
\begin{equation}
\Delta_1= 1 + \frac{(1+r_0)^4}{96 r_0^2}t_2 - \frac{(1+r_0)^4(2+r_0^2+3r_0^4)}{480 r_0^4}t_4
\end{equation}
%
in such a way that for small enough $r_0$ the constraint rules out both positive and negative values for both coefficients, thus leaving us just with Einstein-Hilbert gravity to this order. However if there is a cut-off for the impact parameter such as for example the string length, $l_s$, we would need the third (helicity zero) constraint to close the allowed region for $t_{2,4}$ in such a way that
%
\begin{equation}
t_2  \sim \left(\frac{l_s}{R}\right)^2 \qquad \qquad t_4 \sim \left(\frac{l_s}{R}\right)^4
\end{equation}
% 
where $R$ is the radius of AdS (set to one before). Below that scale we need full string theory to carry out the computation correctly. 
























==> resumo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\chapter{\bfseries \itshape Resumo e conclusi\'ons}
\chaptermark{Resumo e conclusi\'ons}
\label{resumo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{.6cm}

\begin{quotation}
\flushright
{\it ``Was du ererbt von deinen V\"atern hast,\\ Erwirb es, um es zu besitzen.''}

\vspace{.3cm}

Goethe\footnote{O que herdaches dos teus devanceiros, gánao, para que de verdade sexa teu.} 

\end{quotation}

\vspace{3cm}

\noindent As teor\'ias de Lovelock son a extensi\'on natural da Relatividade Xeral en dimensi\'ons superiores a catro. Poden tam\'en ser consideradas coma un modelo de xoguete axeitado para a an\'alise de certos aspectos de teor\'ias con correcci\'ons de orde superior na curvatura libres de {\it pantasmas}. Esas teor\'ias da gravidade capturan algunhas das propiedades caracter\'isticas que definen as gravidades con termos de orde superior, nomeadamente a existencia de máis dun beleiro (A)dS e unha dinámica complexa, solucións de buraco negro máis xerais e ines-tabilidades; evitando así mesmo algúns dos seus problemas. En particular, a gravidade de Lovelock dá lugar a ecuacións de movemento de segunda orde, que polo tanto poden ser consideradas máis aló do réxime perturbativo, e está exenta das pantasmas associadas as derivadas superiores. Isto proporciona un campo de traballo moi atractivo para explorar distintos aspectos gravitacionais e holográficos das teorías con correccións de orde superior na curvatura.

A maioría dos baleiros da teoría teñen buracos negros asociados que presentan características interesantes. Ademais, os buracos negros con horizontes maximalmente simétricos están suxeitos ao teorema de Birkhoff e a correspondente métrica pódese atopar analiticamente. A maioría dos esforzos, na literatura científica adicáronse, con todo, a un determinado sector de solucións, moitas veces restrinxida a unha combinación específica dos coeficientes de Lovelock. O sector ou {\it rama} xeralmente escollido para a análise é a chamada rama de Einstein-Hilbert (EH), xa que de feito, esta se reduce á solución da Relatividade Xeral ao apagar os coeficientes de order superior. Nesta tese presentamos algunhas ferramentas que permiten a descrición de buracos negros de Lovelock con valores arbitrarios de todo o conxunto de parámetros, a  dimensionalidade e a orde da teoría. A pesares do feito de a solución ser implícita, é posíbel extraer a información relevante e discutir toda a posible casuística na situación máis xeral, analizar o número de horizontes, a estabilidade termodinámica da solución, transicións de fase, etc. Ademais, este enfoque ten sido xeneralizado para o caso de solucións cargadas e mesmo cosmolóxicas, e tamén para as chamadas teorías {\it case-topolóxicas}, que comparten a mesma forma das solucións de buraco negro  das gravidades de Lovelock estando definidas en menores dimensións.

Este método é moi útil para gañar intuición sobre procesos físicos que involucran buracos negros. Por poñer un exemplo, é moi doado ilustrar a evolución da posición e número de horizontes a medida que masa da solución varía, o que fornece información crucial sobre a posible aparición de singularidades espidas e a violación da terceira lei da termodinámica. Vimos que a simetría ríxida imposta á solución inxenuamente permite tal comportamento, o que é evitado unha vez a estabilidade da solución é tomada en consideración.

Analizamos a propagación de perturbacións no espazo-tempo definido pola solución  buraco negro ou singularidade espida no límite de momentos e frecuencia altas. Este réxime restrinxido presenta a vantaxe de ser moi simple, ao tempo que suficientemente potente para probar a estabilidade das solucións de interese. Por outra banda, a inestabilidade parece xurdir antes a enerxías altas. Testamos deste xeito as nosas solucións e descubrimos que a inestabilidade aparece  sempre que nos achegarmos á aparición de singularidades espidas, isto é, antes do horizonte do buraco negro desaparecer a solución tórnase inestábel, sendo incerto onde conduce esta inestabilidade. As solucións con singularidades espidas son do mesmo xeito inestábeis, polo que non poden tampouco  ser formadas por colapso. Isto tamén acontece para os casos nos que un inxenuamente agardaría a aparición dun buraco negro extremal (sen carga) e {\it saltos} repentinos da posición do horizonte, preservando entón a terceira lei da termodinámica para as teorías de Lovelock, polo menos para esta clase de buracos negros. 

As mesmas inestabilidades aparecen tamén no proceso de evaporación de buracos negros esféricos nunha gran variedade de situacións. De feito, este comportamento só é evitado por solucións cunha singularidade puntual (tamén as hai de tamaño finito) en dimensións maiores ou iguais a $ 3K + 1 $, sendo $K $ a orde da teoría de Lovelock. A acción de Einstein-Hilbert semella especial a este respecto, xa que é a única teoría de  Lovelock que é estable en cada dimensión na cal pode ser definida. O caso  de dimension tres é especial, xa que a gravidade de Einstein-Hilbert neste caso é unha teoría de Chern-Simons do grupo de AdS, e polo tanto topolóxica. A imaxe global, que xorde a partires desta análise, parece indicar que estas inestabilidades teñen un rol central dinámica gravitatoria. Sen ser unha patoloxía da teoría, como se ten dito nalgunha ocasión, as inestabilidades {\it evitan} a aparición de comportamento  verdadeiramente patolóxico na mesma. Ademais,  impoñen de maneira xenérica un límite superior sobre a {\it  densidade efectiva}, $ M / R^{d-1} $, de calquera obxecto, límite que depende da rama específica da teoría que estamos considerando. Isto semella impedir a existencia de entidades puntuais na maioría dos casos.

Asimesmo, achamos que as transicións de fase de Hawking-Page ocorren de forma xenérica nas teorías  de Lovelock. A única diferenza coa Relatividade Xeral é a posibilidade de ter máis dun burato negro termodinamicamente estábel á mesma temperatura para certos rangos desta última, de tal xeito que a transición pode ocorrer entre dous buracos negros de diferente masa. Por analoxía co caso de Einstein-Hilbert, a transición entre o baleiro térmico  e o buraco negro pode ser identificada como unha transición de confinamento/deconfinamento da CFT dual, en consecuencia, as transicións entre dous buracos negros corresponden a distintas fases deconfinadas  da teoría de campos.

Outra característica aparentemente patolóxica dos buracos negros de Lovelock é a posibilidade de mostrar valores negativos da entropía. Con todo, estes estados problemáticos poden ser evitadas se nos restrinxirmos á fase globalmente preferida para  cada temperatura. Para isto, nalgúns casos, por exemplo buracos negros hiperbólicos, foi crucial ter conside-rado na nosa análise a posibilidade de configuracións extremais con temperatura arbitraria e entropía nula, de acordo cos métodos semi-clásicos. Isto é importante para ter un estado de menor enerxía ou {\it groundstate} ben definido, con masa mínima a calquera temperatura de tal xeito que os estados de entropía negativos teñen sempre unha enerxía libre maior e son así globalmente inestábeis. Isto pode  tamén fornecer información de interese sobre o papel que xogan estes estados extremais e sobre se deben ser considerados só como casos límite dos seus compañeiros non extremais ou a calquera temperatura.

As gravidades de Lovelock amosan unha familia de baleiros -- e as correspondentes solucións de buraco negro -- que suxiren a posibilidade dun diagrama de fases ben complexo. A fin de estudar o diagrama de fases da teoría completa, sen restrinxírmonos a unha rama específica, temos que poder describir a posibilidade de transicións de fase entre as diferentes ramas da teoría. Isto tamén podería ser considerado como un posible desenlace das inestabilidades mencionadas anteriormente. Isto último foi parte da motivación inicial para a nosa análise destas transicións, porén inestabilidades e transicións de fase parecen estar correlacionadas só en situacións moi particulares.

A fin de describir as transicións entre diferentes ramas da teoría, ampliamos o tipo de solucións a ser considerado. Mantendo os mesmos requisitos de simetría  permitimos solucións que, sendo continuas, teñen a primeira derivada discontinua (ou a conexión de spin) nunha determinada superficie. A existencia destas solucións é debida aos momentos da teoría de Lovelock seren multivaluados. As  velocidade poden {\it saltar} en calquera punto sempre que os momentos sexan continuos. Esta continuidade dos momentos canónicos a través da xuntura é debida á ausencia de  materia sobre esta superficie. Con todo, isto non quere dicir que os parámetros de masa das solucións interior e exterior sexan iguais, tendo a {\it burbulla} unha masa efectiva $ M_ + - M_-$. Para configuracións estáticas, sexan estas estábeis ou inestábeis, ademais da masa podemos asignar estes {\it thermalons} valores da temperatura e a entropía. Nós mostramos que a contribución dos termos de superficie na burbulla é tal que a enerxía libre de todo o espazo-tempo toma a forma esperada $ F = M_+-T_+ S $, coa masa e a temperatura, $ M_+ $ e $ T_+ $, correspondentes á solución externa, mentres que a entropía $ S $ permanece sen cambios vindo do horizonte interior. Encontramos, tamén, que as relacións habituais entre as variábeis termodinámicas e mesmo a primeira lei da termodinámica son verificadas. Deste xeito probamos a consistencia da imaxe termodinámica para estas configuracións xeneralizadas.

A única hipótese necesaria para que todo o anterior funcione, é a existencia dun horizonte na rexión interior da burbulla. Por simple que poida parecer, esta condición impón importantes restricións sobre o tipo de configuración que poden ser consideradas. Por exemplo, para topoloxía plana a solución interna ten que pertencer necesariamente á rama EH. Isto implica así mesmo que a termodinámica da mencionada rama (identificada polo seu comportamento asintótico) non é alterada pola existencia destas novas solucións e que calquera {\it salto} de rama (baixo certas condicións) levará necesariamente a este sector. En realidade, o {\it thermalon} é sempre a fase termodinamicamente preferida e, polo tanto, unha burbulla aparece necesariamente, cun buraco negro aloxado no seu interior. Nalgúns casos, con todo, dependendo da elección da asintótica o {\it thermalon} co buraco negro EH regular dentro non existe e a transición non pode ter lugar. Os casos non planares son un pouco máis complexos e xenericamente conlevan unha (ou varias) transicións de fase a temperatura finita. Analizamos  o caso da teoría de Lanczos-Gauss-Bonnet (LGB) en gran detalle. O caso hiperbólico é especial, xa que tamén permite thermalons con asintótica EH, pero só por riba de certo valor crítico do coeficiente LGB.

As condicións de xuntura empregadas para atopar as configuracións de burbulla estáticas, determinan tamén a dinámica das mesmas, nomeadamente a estabilidade da súa posición de equilibrio. No caso da gravidade LGB, a burbulla, sendo inestábel, pode expandirse até acadar a fronteira de AdS en tempo finito, cambiando así a asintótica e as cargas da solución. Isto lembra un pouco ao que ocorre no caso dun {\it quench} onde a enerxía é a temperatura do sistema cambia como resultado do traballo realizado durante a variación das condición de contorno. O mecanismo do {\it thermalon} pode ser considerado como un {\it quench} inducido termodinamicamente, en contraposición a unha acción externa sobre  o sistema. No caso da gravidade LGB con condicións de contorno inestábeis ({\it à la} Boulware-Deser), no caso esférico o baleiro térmico é a fase globalmente estábel a baixa temperatura ao tempo que existe unha temperatura crítica por riba da cal a enerxía libre se volve negativa, indicando a transición. Mesmo para valores positivos da enerxía libre a solución de burbulla existe e pode ser formada cunha probabilidade finita, o sistema dise que é metaestábel. En calquera caso, o sistema é levado necesariamente á rama EH. 

O caso máis interesante é o de topoloxía hiperbólica xa que temos a transición directa (cara a rama EH) con asintótica inestábel pero tamén a inversa con asintótica EH. A situación para a transición directa é moi semellante aos casos esférico e planar,  a transición levando o sistema necesariamente cara asintótica EH.
Con estas outras condicións de contorno, porén, o sistema é estábel para valores moderados do coeficiente LGB xa que non existe ningunha configuración de {\it thermalon} que poida mediar a transición. O espazo-tempo é, polo tanto, necesariamente levado para a rama EH e permanece alí. Para valores máis elevados de $ \lambda $ a situación é abondo distinta con burbullas de ambas fases aparecendo de xeito caótico. Aínda que o buraco negro representa sempre a fase globalmente preferida, as burbullas  teñen unha probabilidade non nula de se formar. Neste caso, a inclusión dos estados extremais a calquera temperatura, parece ser de novo crucial para ter un {\it ensemble} ben definido, polo menos para valores de $\lambda$ pequenos. 

No contexto da correspondencia AdS/CFT os buracos negros corresponden a fases deconfinadas do plasma mentres que a fase confinado é o baleiro térmico. As transicións xeneralizadas de  Hawking-Page mencionadas no parágrafo anterior parecen corresponder a unha transición de fase de confinamento/deconfinamento que inclúen un cambio nas propiedades microscópicas do plasma.


No caso de teorías de Lovelock máis xerais a situación pode cambiar bastante. Por exemplo, o punto de equilibrio de certos {\it thermalons} pode ser estábel, no canto de inestábel, de tal forma que a fase resultante é máis parecida a un buraco negro estándar que aos {\it thermalons} da gravidade LGB. O sistema pode quedar indefinidamente nesa fase se non hai outro {\it thermalon} que leve o sistema a outro lugar. Do punto de vista holográfico, estes {\it thermalons} estábeis constitúen a fase deconfinada de certas ramas da teoría que inxenuamente non terían unha.

As teorías de Lovelock teñen a destacábel característica de que moita información física relevante está codificada no polinomio $ \Upsilon [g] $. As inestabilidades de Boulware-Deser, por exemplo, corresponden  simplemente a $ \Upsilon'[\Lambda] <0 $, o que ten unha fermosa interpretación dual na CFT, a carga central  $ C_T $ ten que ser positiva para a teoría ser unitaria. Nós calculamos a carga central $ C_T $ e puxemos a afirmación anterior en termos concretos, así como os dous parámetros extra, $t_2 $ e $  t_4 $, que aparecen nas funcións de tres puntos do tensor enerxía-impulso. $ t_4 $ é cero no caso particular das teorías de Lovelock, algo que pode estar relacionado con algún tipo de condición de supersimetria da CFT, aínda que a versión supersimétrica das teorías de Lovelock non é coñecida. Tamén discutimos os posíbeis termos que poden contribuír ao cálculo de $t_2 $ e $ t_4 $ no contexto de teorías xerais con correccións de orde superior na curvatura. Restrinxíndonos a termos con ecuacións de segunda orde na solución de {\it shock wave}, há unha correspondencia un a un entre as posíbeis estruturas que aparecen no fluxo de enerxía e as posíbeis correccións de orde superior. Isto tamén coincide co número de combinacións  independentes baixo redefinicións dos campos.

Outra correspondencia ben interesante que foi atopada empregando as teorías de Lovelock é a que relaciona causalidade holográfica en AdS con positividade da enerxía. Ambas condicións físicas son conceptualmente moi diferentes, porén implican o mesmo conxunto de restricións sobre $t_2 $ (con $ t_4 = 0 $). A falta dunha proba definitiva da positividade destes fluxos de enerxía, o anterior pode ser tamén considerado como unha proba indirecta restrinxida ao caso de Lovelock. Ademais, isto levou ao descubrimento de que estas condicións son esixidas pola unitariedade da correspondente CFT \cite{Kulaxizi2011}. Por outra banda, aínda que esta conexión foi descuberta inicialmente para buracos negros, non é unha característica de CFTs térmicas. Realizamos outro cálculo similar, usando unha solución de {\it shock wave} e obtemos restricións equivalentes ás atopadas previamente. Este segundo cálculo tamén deixa claro que o problema ten a súa orixe no vértice de tres gravitóns. Ao contrario das inestabilidades atopadas arriba, a violación de causalidade é unha patoloxía que debe ser descartada coma algo non físico. As inestabilidades porén, poden indicar a existencia de novas solucións ou simplemente ser debidas ao feito de estar expandindo en torno ao baleiro errado. No caso dos buracos negros de Lovelock a estabilidade é necesaria para a validez da solución, non é unha restrición fundamental.

As condicións físicas anteriores restrinxen os posíbeis valores dos coeficientes de Lovelock que describen unha CFT causal. Nótese que esta conexión non tería podido ser descuberta no réxime perturbativo xa que precisamos $ t_2 $  e $  t_4 $ de orde un para que a teoría poida violar causalidade. Ademais, na aproximación de supergravidade $ t_2 $ é da mesma orde que $ \alpha'$ e polo tanto pequeno. Todo isto,  e o feito de que todas as fórmulas parecen estenderse de forma significativa e suave a dimensión e orde da teoría arbitrarias, parece apoiar a idea da aplicabilidade da correspondencia AdS/CFT alén do contexto da teoría das cordas. Aínda que o termo de  Lovelock máis simple aparece en realizacións {\it stringy} da dualidade, os termos de Lovelock de orde superior non foron nunca atopados nese contexto, como tampouco correccións con coeficientes finitos. Entón, teñen as teorías conformes fortemente acopladas cargas centrais necesariamente iguais en catro dimensións? A resposta a esta cuestión non parece ser doada e non atopamos ningún indicio que apunte en calquera dos dous sentidos.

Contrariamente a certas expectativas previas, tamén atopamos que a violación de causa-lidade tamén pode ocorrer no interior da xeometría. Isto mostra ademais que esta patoloxía non está necesariamente ligada ás propiedades ultravioletas da teoría de campos nin a posi-tividade da enerxía en todos os casos, so cando ocorre perto da fronteira de AdS. Sería interesante verificar se este efecto podería estar relacionado coa positividade de funcións de máis puntos dos operadores  fluxo de enerxía.

Finalmente, analizamos as restricións impostas pola causalidade/positividade sobre ou-tras cantidades relevantes da teoría de campos, en particular coeficientes de transporte coma a viscosidade de cisallamento. O cociente desta cantidade con respecto á densidade de entropía, $\eta/s$, é corrixido do seu valor KSS, $ \eta / s = 1/4 \pi $, polo coeficiente de LGB de tal xeito que un límite superior de $ \lambda $ se traduce automaticamente nun límite inferior para $ \eta / s $. A pesares dos termos de Lovelock de orde superior non entraren explicitamente na expresión corrixida de $ \eta / s $, estes si afectan o valor do mínimo. Engaden unha maior liberdade que, consecuentemente, permite a $ \lambda $ tomar valores máis elevados, reducindo desta forma o mínimo de $\eta/s$. Na discusión da existencia ou non dese límite ficou claro que a causalidade por ela mesma non pode impedir a $\eta/s$ tomar valores arbitrariamente pequenos, mesmo negativos nalgúns casos. De feito, é posíbel construír modelos holográficos efectivos onde o termo LGB é orixinado por un VEV doutro campo que condensa no infravermello, isto é so toma valores finitos perto do horizonte sendo cero asintóticamente. Deste xeito, a adición de tal corrección non afecta a causalidade da teoría, ao tempo que modifica o valor da viscosidade. Neste sentido, é posíbel eludir as restricións impostas por causalidade nesta variable. 

Unha vez máis as restricións que evitan os valores non físicos da viscosidade xorden da estabilidade. Despois de todo, a viscosidade negativa tamén corresponde a unha inestabilidade do sistema. Mediante a análise da estabilidade no réxime de altas enerxías, demostramos que $\eta/s$ ten sempre un valor  mínimo distinto de cero independentemente da dimensión ou a order da teoría de Lovelock. Porén, este mínimo redúcese aproximándose a cero a medida que a dimensionalidade $d$ aumenta. Os nosos resultados indican que para valores altos de $ d $, debe ser posible chegar a un valor de $ 4 \pi \eta / s $ de  alomenos $ 1 / K $. Até dez dimensións (\ie orde catro da teoría), pode ser demostrado que o mínimo para cada dimensión segue aproximadamente  unha curva dada por $ 4 \pi \eta / s \approx 1/(d-2) $.

Ao longo desta tese, tentei presentar as teorías Lovelock como un campo de probas interesante de cara a contrastar as nosas ideas sobre a gravidade e a dualidade holográfica. Isto proporcionou información relevante sobre a consistencia e viabilidade das modificacións da acción de Einstein-Hilbert da gravidade e, por contraste, tamén sobre este caso en catro ou máis dimensions. As teorías de Lovelock teñen moitas características interesantes, unha rica dinámica e efectos que non poden ser observados no caso máis simple da Relatividade Xeral. As nosas pescudas desvelaron profundas conexións entre conceptos aparentemente non relacionados. Estas conexións insospeitadas teñen o seu exemplo máis célebre na equivalencia entre causalidade en AdS e a positividade da enerxía na teoría conforme, mas descubrimos exemplos máis sutís. As inestabilidades teñen un papel destacado neste contexto, tanto relacionado coa preservación da Hipótese de  Censura Cósmica ou a terceira lei da mecánica de buracos negros nas gravidades de Lovelock, como co proceso de evaporación dos buracos negros e a existencia dun valor mínimo de $ \eta / s $ nestas teorías. A diversidade das situacións nas que estas inestabilidades desempeñan unha función é moi importante e  merecen unha investigación máis aprofundada. Tamén pode ser interesante investigar as súas implicacións no contexto da correspondencia AdS/CFT, en especial sobre os posibles valores de outros coeficientes de transporte do plasma dual. 


Despois desta longa travesía, as gravidades de Lovelock móstranse como un conxunto complexo e interesante de teorías gravitatorias, non inconsistentes en calquera aspecto fundamental. Porén, hai aínda multitude de avenidas abertas para investigar, moitos problemas sen resolver. Por exemplo, en dimensións maiores que catro hai un incremento enorme na variedade de solucións rotantes, {\it black rings}, {\it black saturns}, multi {\it black rings}, etc. Unha interesante pregunta a ser respondida no contexto das teorías de Lovelock sería até que punto esta rica estrutura pervive. Para iso queda aínda un longo camiño xa que nen sequera se coñece a forma das solucións rotantes máis simples. Outra cuestión non suficientemente explorada é a da reducción dimensional das gravidades de Lovelock, as relacións entre teorías de diferentes  ordes -- en particular coa Relatividade Xeral -- e a estimulante posibilidade da compactificación espontánea destas teorías. Na exploración de novos camiños para simplificar e obter novas perspectivas sobre a dinámica gravitatoria, o límite infinito dimensional ten atraído certa atención. As teorías de Lovelock son a extensión máis obvia tamén a este respecto, xa que fornecen un segundo parámetro, $K$, a orde da teoría, que podería mesmo escalar tan rápido coma a dimensión do espazo-tempo. 
No contexto holográfico, a noción de entropía de entrelazamento atraiu recentemente moita atención e a gravidade de Lovelock parece ser um bo campo de probas tamén neste caso. Finalmente, como xa foi comentado no cerne da tese, as teorías de Lovelock, mediante a correspondencia AdS/CFT, abren unha nova vía para o estudo de CFTs de dimensión arbitraria, das que non se sabe moito. 

Esperamos que as ferramentas e a información recadada na nosa análise sexa de valor no camiño cara entender correccións de orde superior na curvatura de tipo xenérico.
